Downlink Transmission in FBMC-based Massive MIMO with Co-located and Distributed Antennas

This paper introduces a practical precoding method for the downlink of Filter Bank Multicarrier-based (FBMC-based) massive multiple-input multiple-output (MIMO) systems. The proposed method comprises a two-stage precoder, consisting of a fractionally spaced prefilter (FSP) per subcarrier to equalize the channel across each subcarrier band. This is followed by a conventional precoder that concentrates the signals of different users at their spatial locations, ensuring each user receives only the intended information. In practical scenarios, a perfect channel reciprocity may not hold due to radio chain mismatches in the uplink and downlink. Moreover, the channel state information (CSI) may not be perfectly known at the base station. To address these issues, we theoretically analyze the performance of the proposed precoder in presence of imperfect CSI and channel reciprocity calibration errors. Our investigation covers both co-located (cell-based) and cell-free massive MIMO cases. In the cell-free massive MIMO setup, we propose an access point selection method based on the received SINRs of different users in the uplink. Finally, we conduct numerical evaluations to assess the performance of the proposed precoder. Our results demonstrate the excellent performance of the proposed precoder when compared with the orthogonal frequency division multiplexing (OFDM) method as a benchmark.

==> Decentralized.tex <==
\section{Limited back-haul decentralized processing cell-free in uplink and downlink}

In a variety of cell-free applications, it is assumed that the back-haul capacity and central processing unit computation capacity are not adequate to perform all calculations centrally. Thus, each AP performs preliminary calculations and then sends the pre-processed data to the CPU to acquire the final results by a simple operation like averaging or summation. Additionally, by a decentralized approach, it is not required for APs to share the CSI with CPU. Therefore, matched filtering (MF) is the most common approach in this setup. Each AP receives and precodes the data of users that it have in its service set. This set acquired from the antenna selection process.  Hence, the transmit signal of the $i$th AP can be obtained as 
\begin{equation}
x_i[l] = \sum_{m=0}^{M-1} \sum_{n=-\infty}^{ \infty} \sqrt{p_{i,k}}s^i_{m,n} f_{m,n}[l] ,
\label{bbeq_dec}
\end{equation}
where
\be
s^i_{m,n} = \sum_{k \in \psi_i}^{}H_m^{i,k}d_{m,n}^k.
\ee
The received signal at UE $k$ can be obtained as
\be
r_k[l] = \sum_{i=0}^{N-1} x_i[l] \star h_{k,i}[l] + \eta_k[l],
\label{eq:rec_antenna_dec}
\ee
which can expanded as 


Then the
result, $H_{m}^{i,k}* y_{m,n}^i$ is sent to the CPU and CPU takes average over the received values. Thus, at the CPU we have
\begin{equation}
\begin{aligned}
    &\hat{s}_{m,n}^{k} = \mathfrak{R} \big\{\frac{1}{N} \big( \sum\limits_{n' = - \infty}^{\infty} \sum\limits_{i=1}^{N} \sum\limits_{m' = 0}^{M-1} (H_m^{i,k})^* H_{mm',nn'}^{i,k} s_{m',n'}^k + \\
    &\sum_{k' \neq k}^{} \sum\limits_{n' = - \infty}^{\infty} \sum\limits_{i=1}^{N} \sum\limits_{m' = 0}^{M-1}
    (H_m^{i,k})^* H_{mm',nn'}^{i,k'}s_{m',n'}^{k'} \big) \big\}
    \end{aligned}
    \label{decentralized-MRC}
\end{equation}
In the decentralized setup, by following the same procedure of the centralized setup, and using the Tchebyshev theorem, we obtain
\begin{equation}
\begin{aligned}
    &\hat{s}_{m,n}^{k} = \mathfrak{R} \big\{\frac{1}{N} \big( \sum\limits_{n' = - \infty}^{\infty} \sum\limits_{i=1}^{N} \sum\limits_{m' = 0}^{M-1} \mathds{E} \big\{
    (H_m^{i,k})^* H_{mm',nn'}^{i,k} \big\}s_{m',n'}^k \\
    & +\sum_{k' \neq k}^{} \sum\limits_{n' = - \infty}^{\infty} \sum\limits_{i=1}^{N} \sum\limits_{m' = 0}^{M-1}
    \mathds{E}\{(H_m^{i,k})^* H_{mm',nn'}^{i,k'} \big \} s_{m',n'}^{k'} \big) \big\}
    \end{aligned}
    \label{decentralized-MRC2}
\end{equation}
We have to note that noise and channel realization are uncorrelated and this leads to the convergence of the second term and noise related term to zero. Thus, the demodulated symbol in this setup can be represented as
\begin{equation}
\begin{aligned}
    &\hat{s}_{m,n}^{k} = \mathfrak{R} \big\{\frac{1}{N} \big( \sum\limits_{n' = - \infty}^{\infty} \sum\limits_{i=1}^{N} \sum\limits_{m' = 0}^{M-1} \mathds{E} \big\{
    (H_m^{i,k})^* H_{mm',nn'}^{i,k} \big\} s_{m',n'}^k \big) \big\}
    \end{aligned}
    \label{decentralized-MRC3}
\end{equation}
which leads to the same derivations as in centralized cell-free and the equivalent channel can be obtained as
      \be
        g_{mm'}^{k,k'}[n] \rightarrow   
       (f_{m'}[l]  \star  \frac{\sum_{i=0}^{N-1} \beta_{i,k} p^{ik}_m[l]}{N} \star  f_m^*[-l])_{ \downarrow \frac{M}{2}}
       \ee
  Again, the correlation between channel taps and channel impulse response results in a converging equivalent channel to the average of PDPs, and this effect can be modified by using PDP-based equalizers. 
  
  But because of the nature of MRC, the gain in this case in not noticeable compared to the ZF and MMSE combiner in the previous section. The same conclusion made in \cite{aminjavaheri2018filter} for MRC. 

==> Training.tex <==
\color{blue}
\section{Downlink Training}
In the massive MIMO scenarios considered in this work, UE does not have any information on the channel unless a feedback link is added to the model.  Due to the limited channel hardening in setups with moderate or distributed antennas, downlink training can help increase the output of SINR. In the following, we investigate the effects of downlink training in massive MIMO networks with both co-located and distributed antennas. 

\subsection{Co-located}
The theoretical development for the co-located antennas in \ref{sec:calibration} shows that the channel estimation and reciprocity errors reduce to a single scaling factor across all the subcarrier bands. This is a result of statistical averaging among the massive MIMO channels between the BS and each UE. This scaling factor may be found at the receiver if the BS transmits a pilot symbol/signal to each UE. The UE uses this pilot to identify the gain factor, i.e., $\frac{\lambda^2}{(1+{\sigma}_{\rm ef}^2)}$, that should be applied to bring the received signal level to the correct value. It's worth noting, while the BS acquires the statistical information of the channel and uplink reciprocity error, it does not have the downlink imperfect reciprocty information and all these effects can be compensated in the downlink training phase.

This clearly is a simple fix that may be simultaneously applied to all UEs in the network by allocating a single FBMC frame for this purpose or sending a set of scattered pilots in the payload part of each downlink packet. One may note that pilot symbols of different UEs can overlap in time and/or frequency since the precoder conditions the transmit signals such that each UE only receives its associated information-carrying signal. Packets that belong to other UEs are suppressed/nulled. 

It is worth noting in the case of available statistical information at the BS, the statistical compensation results in a better performance compared to the downlink training-based approach. This arises from the fact that a training-based estimation of statistical information does not rely on long-term averaging and infuses error of estimation into the system. This case is equivalent to estimating the statistical parameters in one snapshot. 

\subsection{Distributed/Cell-Free}
In the cell-free scenario, the number of effective antennas is limited. Therefore, detection can not rely on the hardening effect. As studied recently by authors in \cite{interdonato2019downlink}, cell-free shows benefit from pilot more than a co-located setup. In the FBMC-based cell-free massive MIMO setup, as shown by \eqref{eq:MMSEinput_est_cell}, in the presence of large enough effective antennas, the effect of imperfections can be compensated using  the statistical information of errors. Therefore, analogous to a co-located antenna setup, in the cell-free/distributed setup estimation of calibration error effect is enough. In fact, if want to compensate for all the effects in the downlink direction, we need to estimate a multipath channel. 
 By separating the effect of channel estimation and calibration errors, we note that the effect of channel estimation can be compensated in the implementation of the proposed FSP. However, the knowledge of calibration error may not be available at the BS and needs to be acquired in the downlink training. \textcolor{red}{But, as discussed in the co-located part, it is expected to achieve a better performance using a pilot-based compensation on the user side. }

\subsection{Optimum Pilot-aided sequence}
As discussed, in both antenna setups, the downlink training is more practical since imperfection effects show up in the downlink direction. 
Estimation of the equivalent channel would suffice for the acquisition of the total reciprocity calibration error effect, $\lambda$. It is worth noting that this estimation is less complex than a multi-path channel estimation in the uplink, which is required to be performed for every channel between users and antennas.

In a co-located scenario,  one may note that pilot symbols of different UEs can overlap in time and/or frequency since the precoder conditions the transmit signals such that each UE only receives its associated information-carrying signal. Packets that belong to other UEs are suppressed/nulled. Thus, in order to have averaging over noise, a limited number of pilots is enough. Especially, assuming a ZF or MMSE precoder, the effect of multiuser interference vanishes in the large antenna setup, and using a single-user pilot structure suffices this scenario. Our simulation results show the effectiveness of this approach.

\textcolor{red}{In the cell-free setup, the co-located assumptions does not hold. }
	
	

	


